Lattice QCD at finite temperature and density

QCD at finite temperature and density is becoming increasingly important for various experimental programmes, ranging from heavy ion physics to astro-particle physics. The non-perturbative nature of non-abelian quantum field theories at finite temperature leaves lattice QCD as the only tool by which we may hope to come to reliable predictions from first principles. This requires careful extrapolations to the thermodynamic, chiral and continuum limits in order to eliminate systematic effects introduced by the discretization procedure. After an introduction to lattice QCD at finite temperature and density, its possibilities and current systematic limitations, a review of present numerical results is given. In particular, plasma properties such as the equation of state, screening masses, static quark free energies and spectral functions are discussed, as well as the critical temperature and the QCD phase structure at zero and finite density.

==> mu1.tex <==
\section{Lattice QCD at finite density}

Since 2001, significant progress was made towards simulating QCD with realistic parameter values
at small baryon densities. This is achieved by a number of methods that circumvent the sign problem,
rather than solving it: i) Multi-parameter reweighting, ii) Taylor expansion around $\mu=0$ and iii) simulations at imaginary chemical potential, either followed by analytic continuation or Fourier transformed to the canonical ensemble. 
It is important to realize that all of these approaches introduce some degree of approximation. However, their systematics errors are rather different, thus allowing for powerful crosschecks.  
The methods are found to be reliable as long as $\mu/T\lsim 1$, or $\mu_B\lsim 550$ MeV, which includes the region of interest for heavy ion collisions. 

Having developed appropriate computational tools, one can repeat the studies discussed in the
previous sections and see how finite baryon densities affect the screening masses, the equation of state \cite{} or the static potential \cite{}. In all those cases the effect of the chemical potential is found to be rather weak, and for lack of space we will not further discuss those calculations here.
We likewise have to pass over the work done on certain modifications of QCD, for which the sign problem is manageable or absent, such as QCD in the static limit, two-colour QCD or QCD at finite isospin.
Such studies give important qualitative insights and some are covered in previous reviews \cite{latrev}.   
Instead we concentrate here on calculations of the QCD phase diagram at finite density, where qualitative changes are expected for the phase transition as $\mu$ is increased, \fig\ref{fig:1schem}.
More detailed reviews of the same subject can be found in \cite{oprev, csrev}. 

\subsection{The QCD phase diagram for $\mu\neq 0$}

If a chemical potential is switched on for the light quarks, there is an additional parameter requiring
an additional axis for our phase diagram characterizing the order of the transition, \fig\ref{fig:1schem}.
This is shown in \fig\ref{fig:2schem}, where the horizontal plane is spanned by the $\mu=0$ phase diagram in $m_s, m_{u,d}$ and the vertical axis represents $\mu$. 
The critical line separating the first order section from the crossover will now extend to finite $\mu$ and
span a surface. A priori it is, of course, not known whether this surface might be leaning to the right or the left, or even have a more complicated behaviour as a function of the quark masses. 
%
\begin{figure}[t!]
\centerline{
\scalebox{0.65}{\includegraphics{3dphasediag_3.eps}}
\scalebox{0.65}{\includegraphics{3dphasediag_42.eps}}
}
\centerline{
\scalebox{0.58}{\includegraphics{2dphasediag5.eps}}
\scalebox{0.58}{\includegraphics{2dphasediagX5.eps}}
}
%\vspace*{-0.5cm}
%\vspace*{-0.5cm}
\caption{Upper panel: 
The chiral critical surface in the case of positive (left) and negative (right) curvature.
If the physical point is in the crossover region for $\mu=0$, a finite $\mu$
phase transition will only arise in the scenario (left) with positive curvature,
where the first-order region expands with $|\mu|$.
Note that for heavy quarks, the first-order region shrinks with $|\mu|$ (right)
~\cite{Potts}.
%\end{figure*}
%
%
%\begin{figure*}[h!]
Lower panel: phase diagrams for fixed quark mass (here $N_f=3$) corresponding to 
the two scenarios depicted above.}
\end{figure}
%
However, the expected QCD
phase diagram is only obtained if the left situation of \fig\ref{fig:2schem} is realized (unless there are additional critical surfaces yet unknown). 
The first order region expands as $\mu$ is turned on, so that the
physical point, initially in the crossover region, eventually belongs to the
critical surface. At that chemical potential $\mu_E$, the transition is second order:
that is the QCD critical point. Increasing $\mu$ further makes the transition
first order. Drawn in the $(T,\mu)$-plane, this corresponds to the standard
expected phase diagram at the lower left in \fig\ref{2schem}.
A completely different scenario arises if instead the first-order
region shrinks as $\mu$ is turned on. In that case (\fig\ref{fig:2schem} right), the physical
point remains in the crossover region for any $\mu$.

There are now different strategies to determine the QCD phase diagram. One can fix a particular
set of quark masses in the crossover region, and for that theory switch on and increase the chemical potential to see whether a critical surface is crossed or not. This is the approach followed in 
\cite{fk1,fk2,swa1,swa2,gg}. Alternatively, one can start from the known critical line at $\mu=0$
and study its evolution with a finite $\mu$. That will give information on the whole phase diagram
in \fig\ref{fig:2schem}, including, eventually, physical QCD.

\subsection{Two parameter reweighting}

Significant progress enabling finite density simulations was made a few years ago, by a generalisation of the Glasgow method \cite{gla} to reweighting in two parameters \cite{fk0}.  
The partition function is rewritten identically as
\be 
Z=\left \langle \frac{\ex^{-S_g(\beta)}\det(M(\mu))}
{\ex^{-S_g(\beta_0)}\det(M(\mu=0))}\right\rangle_{\mu=0,\beta_0},
\ee
where the ensemble average is now generated at $\mu=0$ and a lattice gauge coupling 
$\beta_0$, while a reweighting factor takes us to the values
$\mu,\beta$ of interest. 
The original Glasgow method reweighted in $\mu$ only and was suffering from the
overlap problem: while the reweighting formula is exact, its Monte Carlo evaluation is not. The integral
gets approximated by a finite number of the most dominant configurations, which are different for the reweighted and the original ensemble, and this difference grows with $\mu$.
When calculating critical behavior at some $\mu$, one-parameter reweighting uses a non-critical ensemble at $\mu=0$, thus missing important dynamics.
By contrast, two-parameter reweighting proceeds along the pseudo-critical line of the phase change, thus always working with an ensemble that probes both phases. This approach produced the first finite density phase diagram from the lattice, obtained for light quarks corresponding to $m_\pi\sim 300$ MeV  \cite{fk1}. A Lee-Yang zero analysis \cite{lyz} was employed in order to find the change from crossover behaviour at $\mu=0$ to a first order transition for $\mu>\mu_c$.  
A later simulation at physical quark masses puts the critical point 
at $\mu_B^c\sim 360$ MeV \cite{fk2}, Fig.~\ref{fk} (left). In this work $L^3\times 4$ lattices with $L=6-12$
were used, working with the standard staggered fermion action and using the R-algorithm. Quark masses were tuned to $m_{u,d}/T_0\approx 0.037, m_s/T_0\approx 1$, corresponding to the mass ratios $m_{\pi}/m_{\rho}\approx 0.19, m_{\pi}/m_K\approx 0.27$, which are close to their physical values.
%
\begin{figure}[t]    
\vspace*{-2cm}
{\rotatebox{0}{\scalebox{0.4}{\includegraphics{phase_diag.eps}}}}\hspace*{1cm}
{\rotatebox{0}{\scalebox{0.75}{\includegraphics{fks.eps}}}}
%\vspace*{-1.5cm}
\caption[]{Left: The phase diagram for physical quark masses as predicted by the two parameter reweighting method \cite{fk2}. Right: High density results from the density of states method for the four-flavour theory, indicating a triple point \cite{cs}. }
\label{fk}
\end{figure}
%

A difficulty in this approach is that the determinant
needs to be evaluated exactly.  Because of the sign problem the reweighting factor is exponentially suppressed with volume and chemical potential, thus limiting the applicability to moderate values of those parameters. This point will be discussed in more detail later.
Moreover, since the statistical fluctuations are those of the simulated ensemble instead of the physical one,  it remains difficult to obtain reliable error estimates. For a proposed procedure see \cite{fk3}. 

Recently, two-parameter reweighting has been combined with the density of states method \cite{dos}, in order to extend the applicability of reweighting to larger values of $\mu/T$ and thus to lower $\mu$. 
First interesting results have been obtained,  indicating a new high density phase and a possible triple point \cite{dos}. Unfortunately, the method is computationally very expensive and so far limited to 
coarse and small lattices, so that it is difficult to systematically affirm those findings at present.

 
\section{Finite density by Taylor expansion}

Another method to gain information about non-zero $\mu$ is to compute the coefficients of a Taylor series expansion of observables in powers of $\mu/T$. 
Early attempts have looked at susceptibilities and the response of screening masses to chemical potential \cite{milc,taro,hlp,gg}. More recently it has also been used to gain information on the phase transition and its nature itself \cite{bisw1}-\cite{ggpd}.
This idea exploits the fact that on finite volumes there are no non-analytic transitions, and hence the partition function $Z(m>0,\mu,T)$ is an analytic function of the parameters of the theory.
For small enough $\mu/T$ one may then hope to get away with only a few terms, whose coefficients are calculated at $\mu=0$. 
Moreover, CP symmetry of the QCD action translates into  a reflection symmetry of the partition function, $Z(\mu)=Z(-\mu)$, such that real physical observables have series expansions in $(\mu/T)^2$. Thus, in particular the pressure density can be expressed as an even power series, 
\be
 p(T,\mu)=-\,\frac{F}{V} 
= \left(\frac TV\right)\log Z(T,\mu),\quad
{p\over T^4}=
\sum_{n=0}^\infty c_{2n}(T) \left({\mu\over T}\right)^{2n}.
\label{press}
\ee
The coefficients are equivalent to generalised quark number susceptibilities at $\mu=0$, and hence measureable with standard simulation techniques.
For high enough temperatures $T>T_0$, the scale of the finite temperature problem is set by the 
Matsubara mode $\sim \pi T$, and one would expect coefficients of order one for an expansion in 
the `natural' parameter $\mu/(\pi T)$ \cite{fp2}. We shall see later that this is indeed borne out by numerical simulations.

Since all the $\mu$-dependence of the partition function is in the fermion determinant, its derivatives  need to be computed,
\be
\frac{\partial \ln \det M}{\partial \mu}  ={\rm tr} \left( M^{-1} \frac{\partial M}{\partial \mu} \right),\quad
\frac{\partial {\rm tr} M^{-1}}{\partial \mu} =
%\hspace{-4mm} = \hspace{-4mm} 
- {\rm tr} \left( M^{-1} \frac{\partial M}{\partial \mu}
 M^{-1} \right), \quad \mbox{etc.},
 \ee
to be iterated for higher orders. These expressions become increasingly complex and methods
to automatize their generation have been devised \cite{ggpd}.
Note that one now is dealing with traces of composite local operators, which greatly facilitates their numerical evaluation by statistical estimators compared to a computation of the full determinant as 
required for reweighting.

If one is interested in phase transitions, finite volume scaling towards the thermodynamic  limit has to be considered. True phase transitions will emerge as non-analyticities, or a finite radius of convergence
for the pressure series. 
If for $\mu=0$ the deconfinement transition is an analytic crossover, one may expand 
about $\mu=0$ and look for the emergence of a finite radius of convergence as the volume increases. 
The radius of convergence of a power series gives the distance between the expansion point and the nearest singularity, and may be extracted from the high order behaviour of the series. A possible 
definition is
\be
\rho = \lim_{n\rightarrow\infty}\rho_n \qquad \mbox{with}\quad
    \rho_n=\left|\frac{c_0}{c_{2n}}\right|^{1/2n}.
%     \qquad
 %  r_n=\left|\frac{c_{2n}}{c_{2n+2}}\right|^{1/2}.
\label{rad}
\ee
General theorems ensure that if the limit exists and asymptotically all coefficients of the series are positive, then there is a singularity on the real axis. 
More details as well as previous applications to strong coupling expansions 
in various spin models can be found in \cite{series}.
In the series for the pressure such a singularity would correspond to the critical point in the $(\mu,T)$-plane.
 
A critical endpoint for the $N_f=2$ theory, based on this approach, was reported  in \cite{ggpd}. The
authors perfomed simulations on $L^3\times 4$ lattices with $L=8-24$, using the standard staggered action and the R-algorithm. The quark mass was fixed in physical units to $m/T_c=0.1$. The aim of the simulations was to bracket the critical point by computing the Taylor coefficients of the quark number susceptibility up to sixth order (i.e.~8th order for the pressure) for various temperatures in the range $T/T_c=0.75-2.15$, and extrapolate to finite $\mu$.
This was done for different lattice volumes in order to get an estimate of finite voulme effects.

The results for the convergence radius Eq.~(\ref{rad}) are shown in Fig.~\ref{ggfig}. A rather strong volume dependence is apparent. While for the smaller $8^3$ lattice the estimators $\rho_n,r_n$ do not seem to converge to a finite radius of convergence, the results on the larger $24^3$ lattice are consistent with settling at a limiting value. The boundary between the two behaviours was observed to occur at $Lm_\pi\approx 5-6$ or $L\approx 16-18$, with larger volumes tending to a smaller radius of convergence. 
%
\begin{figure}[t]
\includegraphics*[height=45mm]{ord1.eps}\hspace*{1cm}
\includegraphics*[height=45mm]{chiqO4O6vT.eps}
\caption[]{Left: Estimators of the radius of convergence $\rho_n$, Eq.~(\ref{rad}), at $T/T_0=0.95$.   
Right: Quark number susceptibility computed through $O(\mu^4)$ (dashed lines) and $O(\mu^6)$ (solid lines) \cite{bisw3}.}
\label{ggfig}
\end{figure}
%
Taking the large volume result at face value and extrapolating to all orders the estimate 
for the location of the critical point is $\mu^c_B/T=1.1\pm 0.2$ at  $T/T_0=0.95$, or 
$\mu_B^c/T_c=1.1\pm 0.2$ \cite{ggpd}.
%, which is in a region where one may still hope for
%the Taylor expansion to converge.

\subsection{The pressure to order $\mu^6$ for $N_f=2$}

Another investigation of the finite density phase diagram of the two-flavour theory was made by
the Bielefeld-Swansea collaboration, also using the Taylor expansion of the pressure. 
This group works with a $16^3\times4$ lattice with p4-improved staggered fermions and a Symanzik-improved Wilson action, simulating with the R-algorithm, 
the quark mass is set to $m/T_0\approx0.4$.  The calculation to order $\mu^4$ was performed in \cite{bisw2} while new results on $\mu^6$ are presented in \cite{bisw3}. The last work also contains detailed discussions of two interesting analytic calculations to compare with,
namely the pressure in high temperature perturbation theory \cite{vuo}, which is going to hold at asymptotically high temperatures, as well as the hadron resonance gas model, which gives a rather good description of the pressure in the confined phase \cite{krt}.

In agreement with \cite{ggpd} and qualitative expectations, their detailed results for the coefficients in the pressure series satisfy $c_6\ll c_4 \ll c_2$ for $T>T_0$, i.e.~one would have coefficients of order one for an expansion in $(\mu/\pi T)$. An impression of the convergence of the series can be obtained by looking at the quark number susceptibility calculated to consecutive orders, as shown in Fig.~\ref{susc}.
 %
%\begin{figure}[t]
%\begin{center}
%\includegraphics*[width=0.45\textwidth]{chiqO4O6vT.eps}
%\end{center}
%\caption[]{Quark number susceptibility computed through $O(\mu^4)$ (dashed lines) and $O(\mu^6)$ (solid lines) \cite{bisw3}.}
%\label{susc}
%\end{figure}
%
For $T\lsim 1.2 T_0$, the series seems to converge rapidly and the $\mu^6$-result is compatible with the one through order $\mu^4$. Around the transition temperature $T_0$, the $\mu^4$-results show a peak emerging with growing $\mu/T_0$, which in \cite{bisw2}  was interpreted as evidence for
a critical point. However, the $\mu^6$ contribution suggests that in this region results do not yet converge,  and the structure is hence not a significant feature of the full pressure.

\subsection{The change of the critical line with $\mu$ \label{sec:crit}}

Rather than fixing to one physical theory and considering the effects of $\mu$, one may ask the question how the chiral critical line in \fig\ref{fig:2schem} changes under the influence of finite $\mu$.
This question was adressed by studying the change with an imaginary chemical potential in 
\cite{fp2,fp3}. The methodology employed is the same as in Sec.~\ref{sec:m1m2c}, i.e.~measurement
of the Binder cumulant of the chiral condensate. The results are summarized in \fig\ref{fig:immu}, left. The chemical potential is found to have almost no influence on $B_4$. 
A lowest-order fit, linear in $a m$ and $(a \mu)^2$, gives the error band \fig\ref{fig:immu}, right, 
corresponding to
\be
a m^c(a \mu) = 0.0270(5) - 0.0024(160) (a \mu)^2
\label{c_prime1}
\ee

Care must be taken for the conversion to physical units. The crucial
point is that, as we increase the chemical potential $\mu_I$, we tune
the gauge coupling $\beta$ upwards to maintain criticality, so that $a(\beta)$
decreases: our observation that $a m^c(\mu_I) \approx const.$ does {\em not}
mean that $m^c(\mu_I) \approx const.$, but that $m^c(\mu_I)$ increases
with $\mu_I$, or {\em decreases} with a real chemical potential $\mu$.
If we express the change of the critical quark mass with chemical potential, in lattice
and continuum units, as
\be
\label{c1prime}
%\frac{a m^c(\mu)}{a m^c(0)} = 1 + c'_1 (a \mu)^2 + ... \\
\frac{a m^c(\mu)}{a m^c(0)} = 1 + \frac{c'_1}{a m^c(0)} (a \mu)^2 + ... \qquad
\frac{m^c(\mu)}{m^c(0)} = 1 + c_1 \left( \frac{\mu}{\pi T} \right)^2 + ...
\label{c1}
\ee
then $c_1$ and $c'_1$ are related by
\be
%c_1 = \frac{\pi^2}{N_t^2} c'_1 + \left( \frac{1}{T_c(m,\mu)} \frac{d T_c(m,\mu)}{d(\mu/\pi T)^2} \right)_{\mu=0}
c_1 = \frac{\pi^2}{N_t^2} \frac{c'_1}{a m^c(0)} + \left( \frac{1}{T_c(m,\mu)} \frac{d T_c(m^c(\mu),\mu)}{d(\mu/\pi T)^2} \right)_{\mu=0}.
\ee
Since $c_1'$ is was observed to be nearly zero, it is the second term that dominates, leading
to an overall negative coefficient $c_1=-0.7(4)$ \cite{fp3}, i.e.
\begin{figure}[t!]
\centerline{
\scalebox{0.62}{\includegraphics{global_ph.eps}}
\scalebox{0.62}{\includegraphics{mc_cons.eps}}
}
\caption{Left: $B_4(am,a\mu_I)$ for different imaginary chemical potentials.
Right: One-sigma error band for the critical mass $a m^c(a \mu_I)$ resulting
from a linear fit.}
\label{fig:immu}
\end{figure}

\begin{figure}
\centerline{
{\includegraphics*[width=0.5\textwidth]{m1m2c_mu0.2.eps}}
\includegraphics*[width=0.45\textwidth]{potts.eps}
}
%\centerline{
%\includegraphics[width=8.0cm]{m1m2c_mu0.0.eps}
%\includegraphics[width=8.0cm]{m1m2c_mu0.2.eps}
%}
\caption{Left: Comparison of the critical line at $\mu=0$ and $a \mu_I = 0.2$.
Right: The critical heavy quark mass separating first order from crossover as a function of $\mu^2$ 
\cite{skim}.}
\end{figure}


%\be
%\frac{m^c(\mu)}{m^c(0)} = 1 - 0.7(4) \left( \frac{\mu}{\pi T} \right)^2 + ...
%\label{c1phys}
%\ee
Taken at face value, this is evidence that, in the $N_f=3$ theory on an $N_t=4$ lattice,
the region of first-order transitions {\em shrinks} as a baryon chemical potential
is turned on, and the ``boring scenario'' of \fig\ref{2schem}, right, is realized.
Similar qualitative conclusions are obtained from simulations of the three flavour theory
with an isospin chemical potential~\cite{DKS_mc}, as well as simulations at imaginary $\mu$
employing Wilson fermions \cite{luo}.

This investigation can be extended to the case of non-degenerate quarks.
\fig{fig:m1m2mu} shows a comparison of the critical line for $\mu=0$  with some critical masses
calculated for a sizeable baryon chemical potential. The data show the same trend as for $N_f=3$: the critical mass is nearly unchanged 
or slightly increasing, {\em in lattice units}. The conversion to \linebreak physical units
proceeds as in the three flavour case.
Since the critical gauge coupling $\beta_0(a \mu_I)$ increases
with $\mu_I$, the coefficient $B$, which is the dominant contribution to $c_1$,
is negative. Together with a very small or slightly negative value for $c'_1$, 
it implies again that the first-order region {\em shrinks} as the baryon chemical
potential is turned on, and the ``exotic scenario'' of Fig.~2, right, is the correct one.

\subsection{The heavy quark limit: Potts model}

Let us finally discuss the upper right corner of Fig.~\ref{schem_2+1}, i.e.~the region towards the pure gauge limit. 
Simulations of quenched QCD at finite baryon number have been done in \cite{quenb}. 
As the quark mass goes to infinity, quarks can be integrated out and QCD reduces to a gauge theory of Polyakov lines. First simulations of this theory with Wilson valence quarks can be found in \cite{nucu}.
At a second order phase transition, universality allows us to neglect the details of gauge degrees of freedom, so the theory should be in the universality class of the 3d three-state Potts model, which is the 3d Ising model. Hence, studying the three-state Potts model should teach us about the behaviour of QCD in the neighbourhood of the critical line separating the quenched first order region from the crossover region.
For large $\mu$ the sign problem in this theory has actually been solved by means of cluster algorithms \cite{clust}. 

Here we are interested in simulations of the three state Potts model atsmall $\mu/T$ \cite{skim}.  In this case, the sign problem is mild enough for brute force simulations at real $\mu$ to be feasible. 
In \cite{skim}, the change of the critical heavy quark mass is determined as a function of real as well as imaginary $\mu$, as shown in Fig.~\ref{potts}. 
Note that $M_c(\mu)$ rises with real chemical potential. i.e.~the first order region in Fig.~\ref{schem_2+1} shrinks as finite baryon density is switched on. This system is thus an example of the non-standard scenario discussed in the previous section. 
This calculation also gives some insight in the problem of analytic continuation: while \fig\ref{potts} clearly endorses the approach in principle, an $O(\mu^8)$-fit was required to reproduce the data
on both sides of $\mu^2=0$. Similar accuracy is difficult to achieve around the chiral line.  

\subsection{Discussion of critical end point results}

\begin{figure}[t]
\centerline{
\scalebox{0.62}{\includegraphics{fooFK.eps}}
\scalebox{0.62}{\includegraphics{fooGG.eps}}
}
\caption{Left: Effect of keeping the quark mass fixed in lattice units in \cite{FK_phys}.
Right: Comparison at finite $\mu$ between the $N_f=2+1$ and the $N_f=2$ theory
considered in \cite{GG}.}
\label{syst}
\end{figure}

The results about the critical surface from Sec.~\ref{sec:crit} appear to be in qualitative contradiction 
with those of Fodor \& Katz~\cite{FK_phys}
and of Gavai \& Gupta~\cite{GG}, which both conclude for the existence of a critical point
$(\mu_E,T_E)$ at small chemical potential $\mu_E/T_E \lsim 1$. 
In considering the reasons for such disagreement, one can easily see that the different data sets
are actually not inconsistent with each other, and the differing pictures can be explained
by standard systematic effects.

Gavai \& Gupta try to infer the location of the critical point by estimating
the radius of convergence of the Taylor expansion of the free energy in $(\mu/\pi T)^2$.
Regardless of the systematic error attached to such an estimate when only 4 Taylor coefficients
are available, the estimate is made for $N_f=2$ only. 
The $(\mu,T)$ phase diagram of this theory might well be qualitatively different
from that of $N_f=2+1$ QCD, as illustrated in \fig\ref{syst} (right). Its critical endpoint point, obtained 
by intersecting a critical surface when going up vertically from the $N_f=2$ quark mass values,
is clearly a long way from the critical endpoint of physical QCD, and nothing follows from the value of one for the other.

Fodor \& Katz obtain Monte Carlo results at $\beta=\beta_c, \mu=0$, and perform
a double reweighting in $(\beta,\mu)$ along the pseudo-critical line $\beta_c(a\mu)$.
By construction, this reweighting is performed at a quark mass fixed {\em in lattice units}:
$a m_{u,d}=\frac{m_{u,d}}{T_c} = const.$. Since the critical temperature $T_c$ decreases 
as they turn on $\mu$, so does their quark mass. This decrease of the quark mass pushes
the transition towards first order, which might be the reason why they find a critical
point at small $\mu$. This effect is illustrated in the sketch Fig.~5, left, where the bent
trajectory \`a la Fodor \& Katz intersects the critical surface, while the vertical line
of constant physics does not.
Put another way, Fodor \& Katz measure the analogue of eq.(\ref{c1prime}) instead of (\ref{c1}).
From their Fig.~1 (Ref.~\cite{FK_phys}), the coefficient $c'_1$ which one would extract
would be essentially zero as that in \cite{fp3}, Sec.~\ref{sec:crit}. 
Taking the variation of $T_c$ with $\mu$
into account could then make a dominant contribution, which could possibly change the results qualitatively towards the non-standard scenario.

Conversely, only the leading order coefficient of $m_c(\mu)$ has been determined
with poor accuracy in \cite{fp3}. The noise might be due to cancelling contributions of higher 
order, alternating in sign. Such contributions would no longer cancel after continuation to real $\mu$,
where every second sign in the series get flipped, and the interpretation of the same data might
lead to a different picture.  

Finally, one should remember that all those investigations have been done using staggered quarks
and on coarse $N_t=4$ lattices only, which for the measurement of the critical temperature turned not to be in the scaling region yet. On the other hand, a robust finding is the high quark mass sensitivity
of the critical point. In light of these circumstances even the qualitative features of the QCD phase 
diagram cannot be regarded as settled, until the methods are sharpened and applied to finer lattices.




==> pdmu.tex <==

\section{The QCD phase diagram for $\mu\neq 0$}

If a chemical potential is switched on for the light quarks, there is an additional parameter requiring
an additional axis for our phase diagram characterizing the order of the transition, \fig\ref{fig:1schem}.
This generalization is shown in \fig\ref{fig:2schem}, with the vertical axis represents $\mu$ and 
the horizontal plane is spanned by the $\mu=0$ phase diagram in $m_s, m_{u,d}$.
The critical line separating the first order section from the crossover will now etend to finite $\mu$ and
correspondingly span a surface. A priori it is, of course, not known how this critical surface will
extend into the $\mu$-direction, e.g.~it could be leaning to the right or the left, or even have a more complicated wiggling behaviour depending on the quark masses. 
%
\begin{figure}[t!]
\centerline{
\scalebox{0.65}{\includegraphics{3dphasediag_3.eps}}
\scalebox{0.65}{\includegraphics{3dphasediag_42.eps}}
}
\centerline{
\scalebox{0.58}{\includegraphics{2dphasediag5.eps}}
\scalebox{0.58}{\includegraphics{2dphasediagX5.eps}}
}
%\vspace*{-0.5cm}
%\vspace*{-0.5cm}
\caption{Upper panel: 
The chiral critical surface in the case of positive (left) and negative (right) curvature.
If the physical point is in the crossover region for $\mu=0$, a finite $\mu$
phase transition will only arise in the scenario (left) with positive curvature,
where the first-order region expands with $|\mu|$.
Note that for heavy quarks, the first-order region shrinks with $|\mu|$ (right)
~\cite{Potts}.
%\end{figure*}
%
%
%\begin{figure*}[h!]
Lower panel: phase diagrams for fixed quark mass (here $N_f=3$) corresponding to 
the two scenarios depicted above.}
\end{figure}
%
However, the standard expectation for the QCD
phase diagram corresponds to the left of \fig\ref{fig:2schem}. 
The first order region expands as $\mu$ is turned on, so that the
physical point, initially in the crossover region, eventually belongs to the
critical surface. At that chemical potential $\mu_E$, the transition is second order:
that is the QCD critical point. Increasing $\mu$ further makes the transition
first order. Drawn in the $(T,\mu)$-plane, this corresponds to the standard
expected phase diagram at the lower left in \fig\ref{2schem}.
A completely different scenario arises if instead the first-order
region shrinks as $\mu$ is turned on. In that case (\fig\ref{fig:2schem} right), the physical
point remains in the crossover region for any $\mu$.

There are now different strategies to determine the QCD phase diagram. One can fix a particular
set of quark masses in the crossover region, and for that theory switch on and increase the chemical potential to see whether a critical surface is crossed or not. This is the approach followed in 
\cite{fk1,fk2,swa1,swa2,gg}. Alternatively, one can start from the now known critical line at $\mu=0$
and study its evolution with a finite $\mu$. That will give information on the whole phase diagram
in \fig\ref{fig:2schem}, including, of course, physical QCD.

\subsection{Two parameter reweighting}

Significant progress enabling finite density simulations was made a few years ago, by a generalisation of the Glasgow method \cite{gla} to reweighting in two parameters \cite{fk0}.  
The partition function is rewritten identically as
\be 
Z=\left \langle \frac{\ex^{-S_g(\beta)}\det(M(\mu))}
{\ex^{-S_g(\beta_0)}\det(M(\mu=0))}\right\rangle_{\mu=0,\beta_0},
\ee
where the ensemble average is now generated at $\mu=0$ and a lattice gauge coupling 
$\beta_0$, while a reweighting factor takes us to the values
$\mu,\beta$ of interest. 
The original Glasgow method reweighted in $\mu$ only and was suffering from the
overlap problem: while the reweighting formula is exact, its Monte Carlo evaluation is not. The integral
gets approximated by a finite number of the most dominant configurations, which are different for the reweighted and the original ensemble, and this difference grows with $\mu$.
When calculating critical behavior at some $\mu$, one-parameter reweighting uses a non-critical ensemble at $\mu=0$, thus missing important dynamics.
By contrast, two-parameter reweighting proceeds along the pseudo-critical line of the phase change, thus always working with an ensemble that probes both phases. This approach produced the first finite density phase diagram from the lattice, obtained for light quarks corresponding to $m_\pi\sim 300$ MeV  \cite{fk1}. A Lee-Yang zero analysis \cite{lyz} was employed in order to find the change from crossover behaviour at $\mu=0$ to a first order transition for $\mu>\mu_c$.  
A later simulation at physical quark masses puts the critical point 
at $\mu_B^c\sim 360$ MeV \cite{fk2}, Fig.~\ref{fk} (left). In this work $L^3\times 4$ lattices with $L=6-12$
were used, working with the standard staggered fermion action and using the R-algorithm. Quark masses were tuned to $m_{u,d}/T_0\approx 0.037, m_s/T_0\approx 1$, corresponding to the mass ratios $m_{\pi}/m_{\rho}\approx 0.19, m_{\pi}/m_K\approx 0.27$, which are close to their physical values.
%
\begin{figure}[t]    
\vspace*{-2cm}
{\rotatebox{0}{\scalebox{0.4}{\includegraphics{phase_diag.eps}}}}\hspace*{1cm}
{\rotatebox{0}{\scalebox{0.75}{\includegraphics{fks.eps}}}}
%\vspace*{-1.5cm}
\caption[]{Left: The phase diagram for physical quark masses as predicted by the two parameter reweighting method \cite{fk2}. Right: High density results from the density of states method for the four-flavour theory, indicating a triple point \cite{cs}. }
\label{fk}
\end{figure}
%

A difficulty in this approach is that the determinant
needs to be evaluated exactly.  Because of the sign problem the reweighting factor is exponentially suppressed with volume and chemical potential, thus limiting the applicability to moderate values of those parameters. This point will be discussed in more detail later.
Moreover, since the statistical fluctuations are those of the simulated ensemble instead of the physical one,  it remains difficult to obtain reliable error estimates. For a proposed procedure see \cite{fk3}. 

Recently, two-parameter reweighting has been combined with the density of states method \cite{dos}, in order to extend the applicability of reweighting to larger values of $\mu/T$ and thus to lower $\mu$. 
First interesting results,  with indications for a possible triple point, are  shown in Fig.~\ref{fk}. 

 
\section{Finite density by Taylor expansion}

Another method to gain information about non-zero $\mu$ is to compute the coefficients of a Taylor series expansion of observables in powers of $\mu/T$. 
Early attempts have looked at susceptibilities and the response of screening masses to chemical potential \cite{milc,taro,hlp,gg}. More recently it has also been used to gain information on the phase transition and its nature itself \cite{bisw1}-\cite{ggpd}.
This idea exploits the fact that on finite volumes there are no non-analytic transitions, and hence the partition function $Z(m>0,\mu,T)$ is an analytic function of the parameters of the theory.
For small enough $\mu/T$ one may then hope to get away with only a few terms, whose coefficients are calculated at $\mu=0$. 
Moreover, CP symmetry of the QCD action translates into  a reflection symmetry of the partition function, $Z(\mu)=Z(-\mu)$, such that real physical observables have series expansions in $(\mu/T)^2$. Thus, in particular the pressure density can be expressed as an even power series, 
\be
 p(T,\mu)=-\,\frac{F}{V} 
= \left(\frac TV\right)\log Z(T,\mu),\quad
{p\over T^4}=
\sum_{n=0}^\infty c_{2n}(T) \left({\mu\over T}\right)^{2n}.
\label{press}
\ee
Since only even terms appear, the coefficients are equivalent to generalised quark number susceptibilities at $\mu=0$, and hence measureable with standard simulation techniques.
For high enough temperatures $T>T_0$, the scale of the finite temperature problem is set by the 
Matsubara mode $\sim \pi T$, and one would expect coefficients of order one for an expansion in 
the `natural' parameter $\mu/(\pi T)$ \cite{fp2}. We shall see later that this is indeed borne out by numerical simulations.

Since all the $\mu$-dependence in the partition function is sitting in the fermion determinant, it is derivatives of the quark matrix that need to be computed,
\be
\frac{\partial \ln \det M}{\partial \mu}  ={\rm tr} \left( M^{-1} \frac{\partial M}{\partial \mu} \right),\quad
\frac{\partial {\rm tr} M^{-1}}{\partial \mu} =
%\hspace{-4mm} = \hspace{-4mm} 
- {\rm tr} \left( M^{-1} \frac{\partial M}{\partial \mu}
 M^{-1} \right), \quad \mbox{etc.},
 \ee
which can be iterated for higher orders. These expressions become increasingly complex and methods
to automatize their generation have been devised \cite{ggpd}.
Note that one now is dealing with traces of composite local operators, which greatly facilitates the numerical evaluation in a simulation compared to a computation of the full determinant.
The numerical estimate of these expressions proceeds by the random noise method (see \cite{} for a discussion), with typically $O(10)-O(100)$ Gaussian noise vectors.  

If one is interested in phase transitions, finite volume scaling towards the thermodynamic  limit has to be considered. True phase transitions will emerge as non-analyticities in the pressure, which is not the case for analytic crossover behaviour. 
Given that in the two flavour theory with finite masses and for $\mu=0$ the deconfinement transition  is an analytic crossover, one may expand about $\mu=0$ and then look for the emergence of a finite radius of convergence as the volume increases. 
The radius of convergence of a power series gives the distance between the expansion point and the nearest singularity, and may be extracted from the high order behaviour of the series. Two possible 
definitions are
\be
\rho,r = \lim_{n\rightarrow\infty}\rho_n,r_n\qquad \mbox{with}\quad
    \rho_n=\left|\frac{c_0}{c_{2n}}\right|^{1/2n},
     \qquad
   r_n=\left|\frac{c_{2n}}{c_{2n+2}}\right|^{1/2}.
\label{rad}
\ee
General theorems ensure that if the limit exists and asymptotically all coefficients of the series are positive, then there is a singularity on the real axis. 
More details as well as previous applications to strong coupling expansions 
in various spin models can be found in \cite{series}.
In the series for the pressure such a singularity would correspond to the critical point in the $(\mu,T)$-plane.
 
The study of finite size scaling of a Taylor series presents a formidable technical task. Since the coefficients are generalised susceptibilities, each of them exhibits non-trivial finite size scaling. The scaling of the individual coefficients, evaluated at $\mu=0$, has to combine to the correct scaling of the finite density pressure given by the sum, thus requiring delicate cancellations between the individual contributions in the large volume limit. Classifications of the behaviour of various generalised susceptibilities are given in \cite{gg2}. 

% For tables use
%\begin{table}
%\caption{Please write your table caption here.}
%\label{tab:1}       % Give a unique label

% For LaTeX tables use
%\begin{tabular}{lll}
%\hline\noalign{\smallskip}
%first & second & third  \\
%\noalign{\smallskip}\hline\noalign{\smallskip}
%number & number & number \\
%number & number & number \\
%\noalign{\smallskip}\hline
%\end{tabular}
%\end{table}
%

A critical endpoint for the $N_f=2$ theory, based on this approach, were reported  in \cite{ggpd}. The
authors perfomed simulations on $L^3\times 4$ lattices with $L=8-24$, using the standard staggered action and the R-algorithm. The quark mass was fixed in physical units to $m/T_0=0.1$. The aim of the simulations was to bracket the critical point by computing the Taylor coefficients of the quark number susceptibility up to sixth order (i.e.~8th order for the pressure) for various temperatures in the range $T/T_0=0.75-2.15$, and extrapolate to finite $\mu$.
This was done for different lattice volumes in order to get an estimate of finite voulme effects.

The results for the convergence radius Eq.~(\ref{rad}) are shown in Fig.~\ref{ggfig}. A rather strong volume dependence is apparent. While for the smaller $8^3$ lattice the estimators $\rho_n,r_n$ do not seem to converge to a finite radius of convergence, the results on the larger $24^3$ lattice are consistent with settling at a limiting value. The boundary between the two behaviours was observed to occur at $Lm_\pi\approx 5-6$ or $L\approx 16-18$, with larger volumes tending to a smaller radius of convergence. It is reassuring that the numerical values for $\rho_n$ and $r_n$ are consistent with each other.
%
\begin{figure}[t]
\includegraphics*[height=45mm]{ord1.eps}\hspace*{1cm}
\includegraphics*[height=45mm]{chiqO4O6vT.eps}
\caption[]{Left: Estimators of the radius of convergence $\rho_n$, Eq.~(\ref{rad}), at $T/T_0=0.95$.   
Right: Quark number susceptibility computed through $O(\mu^4)$ (dashed lines) and $O(\mu^6)$ (solid lines) \cite{bisw3}.}
\label{ggfig}
\end{figure}
%
Taking the large volume result at face value and extrapolating to all orders the estimate 
for the location of the critical point is $\mu^c_B/T=1.1\pm 0.2$ at  $T/T_0=0.95$, or 
$\mu_B^c/T_c=1.1\pm 0.2$ \cite{ggpd}.
%, which is in a region where one may still hope for
%the Taylor expansion to converge.

\subsection{The pressure to order $\mu^6$ for $N_f=2$}

Another investigation of the finite density phase diagram of the two-flavour theory was made by
the Bielefeld-Swansea collaboration, also using the Taylor expansion of the pressure. 
This group works with a $16^3\times4$ lattice with p4-improved staggered fermions and a Symanzik-improved Wilson action, simulating with the R-algorithm, 
the quark mass is set to $m/T_0\approx0.4$.  The calculation to order $\mu^4$ was performed in \cite{bisw2} while new results on $\mu^6$ are presented in \cite{bisw3}. The last work also contains detailed discussions of two interesting analytic calculations to compare with,
namely the pressure in high temperature perturbation theory \cite{vuo}, which is going to hold at asymptotically high temperatures, as well as the hadron resonance gas model, which gives a rather good description of the pressure in the confined phase \cite{krt}.

In agreement with \cite{ggpd} and qualitative expectations, their detailed results for the coefficients in the pressure series satisfy $c_6\ll c_4 \ll c_2$ for $T>T_0$, i.e.~one would have coefficients of order one for an expansion in $(\mu/\pi T)$. An impression of the convergence of the series can be obtained by looking at the quark number susceptibility calculated to consecutive orders, as shown in Fig.~\ref{susc}.
 %
%\begin{figure}[t]
%\begin{center}
%\includegraphics*[width=0.45\textwidth]{chiqO4O6vT.eps}
%\end{center}
%\caption[]{Quark number susceptibility computed through $O(\mu^4)$ (dashed lines) and $O(\mu^6)$ (solid lines) \cite{bisw3}.}
%\label{susc}
%\end{figure}
%
For $T\lsim 1.2 T_0$, the series seems to converge rapidly and the $\mu^6$-result is compatible with the one through order $\mu^4$. Around the transition temperature $T_0$, the $\mu^4$-results show a peak emerging with growing $\mu/T_0$, which in \cite{bisw2}  was interpreted as evidence for
a critical point. However, the $\mu^6$ contribution suggests that in this region results do not yet converge,  and the structure is hence not a significant feature of the full pressure.

\subsection{The change of the critical line with $\mu$ \label{sec:crit}}

Rather than fixing to one physical theory and considering the effects of $\mu$, one may ask the question how the chiral critical line in \fig\ref{fig:2schem} changes under the influence of finite $\mu$.
This question was adressed by studying the change with an imaginary chemical potential in 
\cite{fp2,fp3}. The methodology employed is the same as in Sec.~\ref{sec:m1m2c}, i.e.~measurement
of the Binder cumulant of the chiral condensate. The results are summarized in \fig\ref{fig:immu}, left. The chemical potential is found to have almost no influence on $B_4$. 
A lowest-order fit, linear in $a m$ and $(a \mu)^2$, gives the error band \fig\ref{fig:immu}, right, 
corresponding to
\be
a m^c(a \mu) = 0.0270(5) - 0.0024(160) (a \mu)^2
\label{c_prime1}
\ee

Care must be taken for the conversion to physical units. The crucial
point is that, as we increase the chemical potential $\mu_I$, we tune
the gauge coupling $\beta$ upwards to maintain criticality, so that $a(\beta)$
decreases: our observation that $a m^c(\mu_I) \approx const.$ does {\em not}
mean that $m^c(\mu_I) \approx const.$, but that $m^c(\mu_I)$ increases
with $\mu_I$, or {\em decreases} with a real chemical potential $\mu$.
If we express the change of the critical quark mass with chemical potential, in lattice
and continuum units, as
\be
\label{c1prime}
%\frac{a m^c(\mu)}{a m^c(0)} = 1 + c'_1 (a \mu)^2 + ... \\
\frac{a m^c(\mu)}{a m^c(0)} = 1 + \frac{c'_1}{a m^c(0)} (a \mu)^2 + ... \qquad
\frac{m^c(\mu)}{m^c(0)} = 1 + c_1 \left( \frac{\mu}{\pi T} \right)^2 + ...
\label{c1}
\ee
then $c_1$ and $c'_1$ are related by
\be
%c_1 = \frac{\pi^2}{N_t^2} c'_1 + \left( \frac{1}{T_c(m,\mu)} \frac{d T_c(m,\mu)}{d(\mu/\pi T)^2} \right)_{\mu=0}
c_1 = \frac{\pi^2}{N_t^2} \frac{c'_1}{a m^c(0)} + \left( \frac{1}{T_c(m,\mu)} \frac{d T_c(m^c(\mu),\mu)}{d(\mu/\pi T)^2} \right)_{\mu=0}.
\ee
Since $c_1'$ is was observed to be nearly zero, it is the second term that dominates, leading
to an overall negative coefficient $c_1=-0.7(4)$ \cite{fp3}, i.e.
\begin{figure}[t!]
\centerline{
\scalebox{0.62}{\includegraphics{global_ph.eps}}
\scalebox{0.62}{\includegraphics{mc_cons.eps}}
}
\caption{Left: $B_4(am,a\mu_I)$ for different imaginary chemical potentials.
Right: One-sigma error band for the critical mass $a m^c(a \mu_I)$ resulting
from a linear fit.}
\label{fig:immu}
\end{figure}

\begin{figure}
\centerline{
{\includegraphics*[width=0.5\textwidth]{m1m2c_mu0.2.eps}}
\includegraphics*[width=0.45\textwidth]{potts.eps}
}
%\centerline{
%\includegraphics[width=8.0cm]{m1m2c_mu0.0.eps}
%\includegraphics[width=8.0cm]{m1m2c_mu0.2.eps}
%}
\caption{Left: Comparison of the critical line at $\mu=0$ and $a \mu_I = 0.2$.
Right: The critical heavy quark mass separating first order from crossover as a function of $\mu^2$ 
\cite{skim}.}
\end{figure}


%\be
%\frac{m^c(\mu)}{m^c(0)} = 1 - 0.7(4) \left( \frac{\mu}{\pi T} \right)^2 + ...
%\label{c1phys}
%\ee
Taken at face value, this is evidence that, in the $N_f=3$ theory on an $N_t=4$ lattice,
the region of first-order transitions {\em shrinks} as a baryon chemical potential
is turned on, and the ``boring scenario'' of \fig\ref{2schem}, right, is realized.
Similar qualitative conclusions are obtained from simulations of the three flavour theory
with an isospin chemical potential~\cite{DKS_mc}, as well as simulations at imaginary $\mu$
employing Wilson fermions \cite{luo}.

This investigation can be extended to the case of non-degenerate quarks.
\fig{fig:m1m2mu} shows a comparison of the critical line for $\mu=0$  with some critical masses
calculated for a sizeable baryon chemical potential. The data show the same trend as for $N_f=3$: the critical mass is nearly unchanged 
or slightly increasing, {\em in lattice units}. The conversion to \linebreak physical units
proceeds as in the three flavour case.
Since the critical gauge coupling $\beta_0(a \mu_I)$ increases
with $\mu_I$, the coefficient $B$, which is the dominant contribution to $c_1$,
is negative. Together with a very small or slightly negative value for $c'_1$, 
it implies again that the first-order region {\em shrinks} as the baryon chemical
potential is turned on, and the ``exotic scenario'' of Fig.~2, right, is the correct one.

\subsection{The heavy quark limit: Potts model}

Let us finally discuss the upper right corner of Fig.~\ref{schem_2+1}, i.e.~the region towards the pure gauge limit. 
Simulations of quenched QCD at finite baryon number have been done in \cite{quenb}. 
As the quark mass goes to infinity, quarks can be integrated out and QCD reduces to a gauge theory of Polyakov lines. First simulations of this theory with Wilson valence quarks can be found in \cite{nucu}.
At a second order phase transition, universality allows us to neglect the details of gauge degrees of freedom, so the theory should be in the universality class of the 3d three-state Potts model, which is the 3d Ising model. Hence, studying the three-state Potts model should teach us about the behaviour of QCD in the neighbourhood of the critical line separating the quenched first order region from the crossover region.
For large $\mu$ the sign problem in this theory has actually been solved by means of cluster algorithms \cite{clust}. 

Here we are interested in simulations of the three state Potts model atsmall $\mu/T$ \cite{skim}.  In this case, the sign problem is mild enough for brute force simulations at real $\mu$ to be feasible. 
In \cite{skim}, the change of the critical heavy quark mass is determined as a function of real as well as imaginary $\mu$, as shown in Fig.~\ref{potts}. 
Note that $M_c(\mu)$ rises with real chemical potential. i.e.~the first order region in Fig.~\ref{schem_2+1} shrinks as finite baryon density is switched on. This system is thus an example of the non-standard scenario discussed in the previous section. 
This calculation also gives some insight in the problem of analytic continuation: while \fig\ref{potts} clearly endorses the approach in principle, an $O(\mu^8)$-fit was required to reproduce the data
on both sides of $\mu^2=0$. Similar accuracy is difficult to achieve around the chiral line.  

\subsection{Discussion of critical end point results}

\begin{figure}[t]
\centerline{
\scalebox{0.62}{\includegraphics{fooFK.eps}}
\scalebox{0.62}{\includegraphics{fooGG.eps}}
}
\caption{Left: Effect of keeping the quark mass fixed in lattice units in \cite{FK_phys}.
Right: Comparison at finite $\mu$ between the $N_f=2+1$ and the $N_f=2$ theory
considered in \cite{GG}.}
\label{syst}
\end{figure}

The results about the critical surface from Sec.~\ref{sec:crit} appear to be in qualitative contradiction 
with those of Fodor \& Katz~\cite{FK_phys}
and of Gavai \& Gupta~\cite{GG}, which both conclude for the existence of a critical point
$(\mu_E,T_E)$ at small chemical potential $\mu_E/T_E \lsim 1$. 
In considering the reasons for such disagreement, one can easily see that the different data sets
are actually not inconsistent with each other, and the differing pictures can be explained
by standard systematic effects.

In \cite{ggpd} the authors infer the location of the critical point by estimating
the radius of convergence of the Taylor expansion of the free energy in $(\mu/\pi T)^2$.
Regardless of the systematic error attached to such an estimate when only 4 Taylor coefficients
are available, the estimate is made for $N_f=2$ only. 
The $(\mu,T)$ phase diagram of this theory might well be qualitatively different
from that of $N_f=2+1$ QCD, as illustrated in \fig\ref{syst} (right). Its critical endpoint point, obtained 
by intersecting a critical surface when going up vertically from the $N_f=2$ quark mass values,
is clearly a long way from the critical endpoint of physical QCD, and nothing follows from the value of one for the other.

In \cite{fk2} Monte Carlo results are obtained at $\beta=\beta_c, \mu=0$, and 
double reweighted in $(\beta,\mu)$ along the pseudo-critical line $\beta_c(a\mu)$.
By construction, this reweighting is performed at a quark mass fixed {\em in lattice units}:
$a m_{u,d}=\frac{m_{u,d}}{T_c} = const.$. Since the critical temperature $T_c$ decreases 
as they turn on $\mu$, so does their quark mass. This decrease of the quark mass pushes
the transition towards first order, which might be the reason why they find a critical
point at small $\mu$. This effect is illustrated in the sketch Fig.~5, left, where the bent
trajectory \`a la Fodor \& Katz intersects the critical surface, while the vertical line
of constant physics does not.
Put another way, Fodor \& Katz measure the analogue of eq.(\ref{c1prime}) instead of (\ref{c1}).
From their Fig.~1 (Ref.~\cite{FK_phys}), the coefficient $c'_1$ which one would extract
would be essentially zero as that in \cite{fp3}, Sec.~\ref{sec:crit}. 
Taking the variation of $T_c$ with $\mu$
into account could then make a dominant contribution, which could possibly change the results qualitatively towards the non-standard scenario.

Conversely, only the leading order coefficient of $m_c(\mu)$ has been determined
with poor accuracy in \cite{fp3}. The noise might be due to cancelling contributions of higher 
order, alternating in sign. Such contributions would no longer cancel after continuation to real $\mu$,
where every second sign in the series get flipped, and the interpretation of the same data might
lead to a different picture.  

Finally, one should remember that all those investigations have been done using staggered quarks
and on coarse $N_t=4$ lattices only, which for the measurement of the critical temperature turned not to be in the scaling region yet. On the other hand, a robust finding is the high quark mass sensitivity
of the critical point. In light of these circumstances even the qualitative features of the QCD phase 
diagram cannot be regarded as settled, until the methods are sharpened and applied to finer lattices.

\section{Conclusions}

We have attempted to summarize our current understanding of finite temperature and density QCD
from numerical studies on the lattice. 
While many of the results in the pure gauge theory are
available in the continuum limit, simulations with
dynamical fermions still suffer from systematic errors.
These are mainly due to finite lattice spacing as well as quark masses
which don't meet their physical values yet.
Nevertheless, for critical temperatures and the equation
of state these problems are now being tackled and the first continuum extrapolations
become available.

Apart from the basic thermodynamic quantities, existing results
provide us with a detailed picture
of how static quantities change through the deconfinement
transition up to a few $T_c$.
Combinations of perturbative calculations and numerical
simulations have produced insight into the regime of very high
temperatures as well as the dynamics
and mixing of modes.
Altogether this lead to a quantitative understanding of the relevant
static length scales in the plasma, as well as tests of the applicability
and breakdown of thermal perturbation theory.

The naive picture of the deconfined phase as a weakly interacting
parton gas is not supported. For temperatures relevant to
heavy ion collisions, the plasma displays strong residual interactions
through soft gluonic modes, which cannot be treated
perturbatively, and which influence different
quantities in different ways. In particular the constituents
themselves are objects dressed by non-perturbative
interactions. This gives a consistend explanation to the
various observed features: the equation of state,
susceptibilities and fermionic correlators
are dominated by hard modes and not far
from their ideal gas values. Gluonic correlators, on the other hand,
are dominated by soft modes and entirely off their leading perturbative
predictions. An ideal gas is established
only at asymptotically high temperatures.

Significant progress was made over the last five years regarding dynamical quantities
as well as finite density simulations. In both fields methods have been developed, that
are currently being scrutinised for their reliability. Calculations of spectral functions provide
an intriguing picture of remnant binding forces in the plasma phase as well as first semi-quantitative
results for the transport coefficients. Calculations at finite density are now possible for $\mu/T\lsim 1$,
with good agreement between all methods whenever equal parameter sets are compared.
However, the way to a quantitative understanding of the QCD phase diagram is still long, mainly due to
the high quark mass sensitivity of the critical endpoint, which requires enormous accuracy in the continuum limit.

